A Strongly Parametrized Mass Ratio Model for the Stable Mass Transfer Channel: a Case Study of the $10 \, \rm{M}_{\odot}$ Peak

The mass ratio of merging binary black holes (BBHs) carries information about their formation history, yet has received less attention than masses, spins and eccentricities as a channel discriminator. We derive a strongly parametrized analytical model for the mass-ratio distribution expected from the stable mass transfer (SMT) channel. The model maps mass-transfer stability and accretion efficiency onto the observed mass-ratio distribution, and naturally produces two qualitatively distinct subpopulations: a non-mass-ratio-reversed and a mass-ratio-reversed subpopulation whose distinct shapes depend on the binary-evolution parameters in a traceable way. We embed this model in a hierarchical population analysis and apply it to the $\sim 10\, \rm{M}_{\odot}$ peak in the GWTC-4 BBH catalog. We find that the data favor little to no mass-ratio reversal in this peak, and infer SMT parameters in an astrophysically plausible range. This work demonstrates how data-driven models can be used in mixtures to study singular features in BBH population data and serves as a proof of concept for how a measurement of the BBH mass-ratio distribution within a subpopulation can be translated into direct constraints on the binary-evolution physics that produced it.

==> macros.tex <==
\makeatletter%
\newcommand\macros[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@out{%
    \{%
      "peak\_location": \{%
        "median": "10.1", %
        "error plus": "1.1", %
        "error minus": "0.74", %
        "5th percentile": "9.3", %
        "95th percentile": "11"%
      \}, %
      "f\_smt": \{%
        "median": "68.6", %
        "error plus": "13.3", %
        "error minus": "24.2", %
        "5th percentile": "44.3", %
        "95th percentile": "81.8"%
      \}, %
      "f\_background": \{%
        "median": "31.4", %
        "error plus": "24.2", %
        "error minus": "13.3", %
        "5th percentile": "18.2", %
        "95th percentile": "55.7"%
      \}, %
      "zeta\_eff\_mrr\_threshold": "4.74", %
      "mrr\_posterior\_percent": "14.3", %
      "no\_mrr\_posterior\_percent": "85.7", %
      "zeta\_eff": \{%
        "median": "4.3", %
        "error plus": "1.9", %
        "error minus": "0.89", %
        "5th percentile": "3.4", %
        "95th percentile": "6.2"%
      \}, %
      "zeta\_eff\_mrr\_only": \{%
        "median": "5.8", %
        "error plus": "0.94", %
        "error minus": "1.1", %
        "5th percentile": "4.7", %
        "95th percentile": "6.7"%
      \}, %
      "zeta\_eff\_no\_mrr\_only": \{%
        "median": "4.2", %
        "error plus": "0.47", %
        "error minus": "0.82", %
        "5th percentile": "3.4", %
        "95th percentile": "4.7"%
      \}, %
      "beta\_acc": \{%
        "median": "0.30", %
        "error plus": "0.23", %
        "error minus": "0.18", %
        "5th percentile": "0.12", %
        "95th percentile": "0.53"%
      \}, %
      "beta\_acc\_mrr\_only": \{%
        "median": "0.43", %
        "error plus": "0.27", %
        "error minus": "0.20", %
        "5th percentile": "0.23", %
        "95th percentile": "0.70"%
      \}, %
      "beta\_acc\_no\_mrr\_only": \{%
        "median": "0.28", %
        "error plus": "0.21", %
        "error minus": "0.18", %
        "5th percentile": "0.11", %
        "95th percentile": "0.50"%
      \}%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{peak_location}=0%
      \let\macros@out\macros@I%
    \else%
      \ifnum\pdfstrcmp{#1}{f_smt}=0%
      \let\macros@out\macros@II%
    \else%
      \ifnum\pdfstrcmp{#1}{f_background}=0%
      \let\macros@out\macros@III%
    \else%
      \ifnum\pdfstrcmp{#1}{zeta_eff_mrr_threshold}=0%
      \def\macros@out{%
    4.74}%
    \else%
      \ifnum\pdfstrcmp{#1}{mrr_posterior_percent}=0%
      \def\macros@out{%
    14.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{no_mrr_posterior_percent}=0%
      \def\macros@out{%
    85.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{zeta_eff}=0%
      \let\macros@out\macros@IV%
    \else%
      \ifnum\pdfstrcmp{#1}{zeta_eff_mrr_only}=0%
      \let\macros@out\macros@V%
    \else%
      \ifnum\pdfstrcmp{#1}{zeta_eff_no_mrr_only}=0%
      \let\macros@out\macros@VI%
    \else%
      \ifnum\pdfstrcmp{#1}{beta_acc}=0%
      \let\macros@out\macros@VII%
    \else%
      \ifnum\pdfstrcmp{#1}{beta_acc_mrr_only}=0%
      \let\macros@out\macros@VIII%
    \else%
      \ifnum\pdfstrcmp{#1}{beta_acc_no_mrr_only}=0%
      \let\macros@out\macros@IX%
    \else%
      \def\macros@out{%
    ??}%
    \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
  \fi
  \macros@out
}\newcommand\macros@I[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@I@out{%
    \{%
      "median": "10.1", %
      "error plus": "1.1", %
      "error minus": "0.74", %
      "5th percentile": "9.3", %
      "95th percentile": "11"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\macros@I@out{%
    10.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\macros@I@out{%
    1.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\macros@I@out{%
    0.74}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\macros@I@out{%
    9.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\macros@I@out{%
    11}%
    \else%
      \def\macros@I@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \macros@I@out
}\newcommand\macros@II[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@II@out{%
    \{%
      "median": "68.6", %
      "error plus": "13.3", %
      "error minus": "24.2", %
      "5th percentile": "44.3", %
      "95th percentile": "81.8"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\macros@II@out{%
    68.6}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\macros@II@out{%
    13.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\macros@II@out{%
    24.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\macros@II@out{%
    44.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\macros@II@out{%
    81.8}%
    \else%
      \def\macros@II@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \macros@II@out
}\newcommand\macros@III[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@III@out{%
    \{%
      "median": "31.4", %
      "error plus": "24.2", %
      "error minus": "13.3", %
      "5th percentile": "18.2", %
      "95th percentile": "55.7"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\macros@III@out{%
    31.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\macros@III@out{%
    24.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\macros@III@out{%
    13.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\macros@III@out{%
    18.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\macros@III@out{%
    55.7}%
    \else%
      \def\macros@III@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \macros@III@out
}\newcommand\macros@IV[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@IV@out{%
    \{%
      "median": "4.3", %
      "error plus": "1.9", %
      "error minus": "0.89", %
      "5th percentile": "3.4", %
      "95th percentile": "6.2"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\macros@IV@out{%
    4.3}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\macros@IV@out{%
    1.9}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\macros@IV@out{%
    0.89}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\macros@IV@out{%
    3.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\macros@IV@out{%
    6.2}%
    \else%
      \def\macros@IV@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \macros@IV@out
}\newcommand\macros@V[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@V@out{%
    \{%
      "median": "5.8", %
      "error plus": "0.94", %
      "error minus": "1.1", %
      "5th percentile": "4.7", %
      "95th percentile": "6.7"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\macros@V@out{%
    5.8}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\macros@V@out{%
    0.94}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\macros@V@out{%
    1.1}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\macros@V@out{%
    4.7}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\macros@V@out{%
    6.7}%
    \else%
      \def\macros@V@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \macros@V@out
}\newcommand\macros@VI[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@VI@out{%
    \{%
      "median": "4.2", %
      "error plus": "0.47", %
      "error minus": "0.82", %
      "5th percentile": "3.4", %
      "95th percentile": "4.7"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\macros@VI@out{%
    4.2}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\macros@VI@out{%
    0.47}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\macros@VI@out{%
    0.82}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\macros@VI@out{%
    3.4}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\macros@VI@out{%
    4.7}%
    \else%
      \def\macros@VI@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \macros@VI@out
}\newcommand\macros@VII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@VII@out{%
    \{%
      "median": "0.30", %
      "error plus": "0.23", %
      "error minus": "0.18", %
      "5th percentile": "0.12", %
      "95th percentile": "0.53"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\macros@VII@out{%
    0.30}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\macros@VII@out{%
    0.23}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\macros@VII@out{%
    0.18}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\macros@VII@out{%
    0.12}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\macros@VII@out{%
    0.53}%
    \else%
      \def\macros@VII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \macros@VII@out
}\newcommand\macros@VIII[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@VIII@out{%
    \{%
      "median": "0.43", %
      "error plus": "0.27", %
      "error minus": "0.20", %
      "5th percentile": "0.23", %
      "95th percentile": "0.70"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\macros@VIII@out{%
    0.43}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\macros@VIII@out{%
    0.27}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\macros@VIII@out{%
    0.20}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\macros@VIII@out{%
    0.23}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\macros@VIII@out{%
    0.70}%
    \else%
      \def\macros@VIII@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \macros@VIII@out
}\newcommand\macros@IX[1][all]{%
  \ifnum\pdfstrcmp{#1}{all}=0%
    \def\macros@IX@out{%
    \{%
      "median": "0.28", %
      "error plus": "0.21", %
      "error minus": "0.18", %
      "5th percentile": "0.11", %
      "95th percentile": "0.50"%
    \}}%
  \else%
    \ifnum\pdfstrcmp{#1}{median}=0%
      \def\macros@IX@out{%
    0.28}%
    \else%
      \ifnum\pdfstrcmp{#1}{error plus}=0%
      \def\macros@IX@out{%
    0.21}%
    \else%
      \ifnum\pdfstrcmp{#1}{error minus}=0%
      \def\macros@IX@out{%
    0.18}%
    \else%
      \ifnum\pdfstrcmp{#1}{5th percentile}=0%
      \def\macros@IX@out{%
    0.11}%
    \else%
      \ifnum\pdfstrcmp{#1}{95th percentile}=0%
      \def\macros@IX@out{%
    0.50}%
    \else%
      \def\macros@IX@out{%
    ??}%
    \fi\fi\fi\fi\fi
  \fi
  \macros@IX@out
}%
\makeatother%
